Proceedings of the workshop: HERA and the LHC workshop series on the implications of HERA for LHC physics

2nd workshop on the implications of HERA for LHC physics. Working groups: Parton Density Functions Multi-jet final states and energy flows Heavy quarks (charm and beauty) Diffraction Cosmic Rays Monte Carlos and Tools

==> include-mc-test.tex <==
\newcommand{\genname}[1]{\texttt{\textbf{#1}}}
\newcommand{\alpgen}{\genname{AlpGen}}
\newcommand{\sherpa}{\genname{SHERPA}}
\chapter[\large  WG: Monte Carlo and Tools]{ Working Group \\ Monte Carlo and Tools}
{\Large\bfseries Convenors:}
\vspace{10mm}

{\Large\itshape
%M. Grothe (CERN), \\
%M. Albrow (FNAL), \\
%K. Werner (Nantes)}

\CLDP
\begin{papers} % start of individual articles/papers



%\coltoctitle{Toolkit for High Energy Physics Event Generation}
 \coltoctitle{{\boldmath\sc ThePEG} Toolkit for High Energy Physics Event Generation}
 \coltocauthor{L. L\"onnblad}
\Includeart{\CAUT}{\CTIT}{WGmc/leif_lonnblad/thepeg}

 \coltoctitle{CASCADE}
 \coltocauthor{M. Deak, H. Jung, K. Kutak}
 \Includeart{\CAUT}{\CTIT}{WGmc/jung/cascade}


 %\coltoctitle{Second Talk}
 %\coltocauthor{David Summerset}
 %\Includeart{\CAUT}{\CTIT}{summerset_david}



\end{papers} % end of individual articles/papers

